Online Control with Adversarial Disturbances

We study the control of a linear dynamical system with adversarial disturbances (as opposed to statistical noise). The objective we consider is one of regret: we desire an online control procedure that can do nearly as well as that of a procedure that has full knowledge of the disturbances in hindsight. Our main result is an efficient algorithm that provides nearly tight regret bounds for this problem. From a technical standpoint, this work generalizes upon previous work in two main aspects: our model allows for adversarial noise in the dynamics, and allows for general convex costs.

==> A-ons.tex <==



\section{ONS for OCO with Memory}


\subsection{Setting, Notation and Algorithm}

We consider OCO with loss functions with memory $f_t(x_t,...,x_{t-m})$. The goal is policy regret, i.e. 
$$ \sum_t f_t(x_t,...,x_{t-m}) - \min_{x^*} \sum_t f_t(x^*,...,x^*) $$
We assume:
\begin{enumerate}
    \item the loss functions are convex for a fixed $x$, i.e. the following functions are convex:
    $$ \ftil_t (x) = f_t(x,...,x)$$
    
    \item  the functions $\ftil_t$ are $\alpha$-exp-concave
    \item The functions $\ftil$ are $L$ Lipschitz, i.e. 
    $$ \ftil_t(x) - \ftil_t(y) \leq L \| x-y\| $$
\end{enumerate}

The algorithm is ONS on the functions $\ftil_t$.


\subsection{main theorem} 
 

\begin{lemma}
Let $\{ f_t \}_{t=1}^T$ be Lipschitz continuous loss functions with memory (from $\mathcal{K}^{m+1}$ to $[0,1]$). Then, ONS over $\{\ftil_t\}$ generates an online sequence $\{ x_t \} _{t=1}^T $, for which the following holds:
\begin{equation*}
R_{T,m} = \sum_{t=m}^T f_t (x_{t-m}, \ldots , x_{t})   -    \min_{x \in \mathcal{K}} \sum_{t=m}^T f_t (x,\ldots,x) = O ( \frac{m^2}{1+G^2}  \log T) .
\end{equation*}
\end{lemma}

\begin{proof}
First, note that applying ONS to the loss functions $\{ f_t\}_{t=1}^T$ is equivalent to applying ONS to the loss functions $\{\tilde{f}_t\}_{t=1}^T$. I.e., given $m$ initial points $ x_1, \ldots, x_m $, both algorithms generate the same sequence of decisions $\{ x_t\}_{t=m}^T$, for which it holds that:
$$
\sum_{t=m}^T \tilde{f}_t (x_{t})   -    \min_{x\in \mathcal{K}} \sum_{t=m}^T \tilde{f}_t (x) = O(\log T) 
$$
or equivalently:
\begin{equation} \label{reg_rftl}
\sum_{t=m}^T f_t (x_{t}, \ldots , x_{t})   -    \min_{x\in \mathcal{K}} \sum_{t=m}^T f_t (x,\ldots,x) = O(\log T) 
\end{equation}
due to the regret guarantee in Theorem \ref{thm:ONS-LMS}.
On the other hand, ${f}_t$ is $L$-Lipschitz continuous, thus 
\begin{eqnarray*}
\left| f_t (x_t,\ldots,x_t)  -  f_t (x_{t-m}, \ldots , x_{t}) \right|  &\leq &  L  \| (x_t,\ldots,x_t) - (x_{t-m}, \ldots , x_{t}) \| \\
& = & L \cdot \sum_{j=1}^{m} \| x_t - x_{t-j} \|  \\
& \leq &  L \cdot \sum_{j=1}^{m}  \sum_{l=1}^{j}  \| x_{t-l+1} - x_{t-l}\|  \\
& \leq & L \sum_{j=1}^{m}  \sum_{l=1}^{j}  \| A_{t-l}^{-1} \nabla_{t-l} \| 
\end{eqnarray*}
where the last inequality follows from definition of ONS and the projection operation. 
Summing over $t=m,\ldots,T$ we get that
\begin{equation} \label{lip_rftl}
\left| \sum_{t=m}^T f_t (x_{t}, \ldots , x_{t}) - \sum_{t=m}^T f_t (x_{t-m}, \ldots , x_{t}) \right|   \leq m^2   \sum_t \| A_{t}^{-1} \nabla_t \| = m^2   \sum_t \| A_{t}^{-1} \frac{{\nabla}_t}{\|\nabla_t\|}  \| \cdot \|\nabla_t\| .
\end{equation}
Next, we need the following claim
\begin{claim}
For any PSD matrix, and unit norm vector $v$, we have 
$$v^\top A^2 v \leq     (v^\top A v)^2   $$
\end{claim}
\begin{proof}
To see this, notice that by rotation it suffices to prove for diagonal matrices, and thus for non-negative numbers $d_i$ that $\sum_i v_i^2 d_i^2 \leq (\sum_i v_i^2 d_i)^2 $, where $\sum_i v_i^2 = 1$. In other words, it suffices to prove that $\E_i[ d_i^2] \leq \E_i[ |d_i| ]^2 $. This follows since the $\ell_2$ norm of a vector is smaller than $\ell_1$ norm. 
\end{proof}
This claim implies in our context that: (let $\tilde{\nabla} = \frac{\nabla}{\|\nabla\|} $)
$$ \| A_t^{-1} \tilde{\nabla}_t  \| = \sqrt{ \tilde{\nabla}_t^\top A_t^{-2} \tilde{\nabla}_t } \leq  ( \tilde{\nabla}_t A_t^{-1} \tilde{\nabla}_t)^2 $$ 

It follows from the vector harmonic series that 
$$ \sum_t (\nabla_t^\top A_t \nabla_t)^2 \leq \sum_t \nabla_t^\top A_t \nabla_t =  O(d \log T)$$
and this implies our theorem.  We may need to use a Newton algorithm that uses the normalized gradients instead of real gradients, for the movement bound to hold.
\end{proof}





\section{An online Newton algorithm} 
 
The algorithm below is a generic Newton algorithm which does not depend on the gradient bounds and/or strong convexity. 



\begin{algorithm}
\caption{Online Newton Step for square loss }
\label{alg:ons-lds}
\begin{algorithmic}[1]
\STATE Input: time horizon $T$, initialization $\delta > 0$. 
\STATE Initialize $\beta_1$, and $A_{0} = \delta I$. 
\FOR{$t = 1, \ldots, T$}
\STATE Observe $f_t = (x^\top a_t -b_t)^2$.  Let $\nabla_{t} = \nabla f_t(x_t)$,  denote the Hessians similarly. 
\STATE Update $x_t$ via the ONS rule, and project:
\[ x_{t+1} \leftarrow  \prod_{\K}^{A_t} \left(  x_t -  A_{t}^{-1} \nabla_{t}    \right)  \ , \ A_{t+1} = A_{t} + \nabla^2_{t}    .\]
\ENDFOR
\end{algorithmic}
\end{algorithm}


For this algorithm, we can show:
\begin{theorem} \label{thm:ONS-LMS}
The regret of Algorithm \ref{alg:ons-lds}  is bounded by 
$$  \sum_t f_t(x_t) \leq \min_{x \in \K} f_t(x)  + d B^2 \log (DT)   $$
where $B$ is an upper bound on function value, and $D = \|x_1 - x^*\| $. 
\end{theorem}


\begin{proof}
Following  standard analysis,
\begin{eqnarray*}
\| x_{t+1} - x^*\|_{A_t}^2 & = \| x_t - A_t^{-1} \nabla_t - x^* \|_{A_t}^2 \\
& = \|x_t - x^* \|_{A_t}^2 - 2 \nabla_t ^\top A_t^{-1} A_t (x_t - x^*) + \nabla_t A_t^{-1} A_t A_t^{-1} \nabla _t  
\end{eqnarray*}
Thus,
 \[ 2 \grad_t^\top(x_t-x^*) \leq \grad_t^\top A_t^{-1} \grad_t +  \|x_t - x^* \|_{A_t}^2 -  \|x_{t+1} - x^* \|_{A_t}^2\]
 Summing over $t=1,\dots,T$, we have
 \begin{align*}
 \sum\limits_{t=1}^T 2 \grad_t^\top (x_t-x^*) &\leq \sum\limits_{t=1}^T \grad_t^\top A_t^{-1} \grad_t +  \|x_1 - x^* \|_{A_1}^2 + \sum\limits_{t=2}^T  \|x_t - x^* \|_{A_t - A_{t-1} }^2 -  \|x_{T+1} - x^* \|_{A_T}^2 \\
&\leq \sum\limits_{t=1}^T \grad_t^\top A_t^{-1} \grad_t +  \|x_1 - x^* \|_{A_1}^2 + \sum\limits_{t=2}^T  \|x_t - x^* \|_{\nabla_t^2 }^2  \\
 \end{align*}
Next, we use the fact that for the square loss, the Hessian is always constant, and have 
 \begin{align*}
 \sum\limits_{t=1}^T f_t(x_t) - f_t(x^*) & =  \grad_t^\top (x_t-x^*) - \frac{1}{2}\sum\limits_{t=1}^T \| x_t - x^*\|_{\hess_t}^2 & \mbox{important!}\\
 & \leq \frac{1}{2} \sum\limits_{t=1}^T \grad_t^\top A_t^{-1} \grad_t +    \frac{1}{2} \| x_1 - x^*\|^2 _{A_1 - \hess_1}
 \end{align*}
Taking $A_0 = \delta I$ for very small $\delta$, we have 
\begin{eqnarray*}
\regret & \leq  \frac{1}{2} \sum\limits_{t=1}^T \grad_t^\top A_t^{-1} \grad_t + \delta \|x_t - x^*\|^2 \\
&  = \frac{1}{2} \sum\limits_{t=1}^T A_t^{-1} \bullet \grad_t \grad_t^\top  + \delta D^2 \\
&  = \frac{1}{2} \sum\limits_{t=1}^T A_t^{-1} \bullet (A_t - A_{t-1} ) \cdot {f_t(x_t)^2}  + \delta D^2 \\
& \leq \frac{B^2}{2} \sum\limits_{t=1}^T \log \frac { |A_t|}{|A_{t-1}|}  + \delta D^2 \\
&\leq  {B^2 d} \log \frac{T}{\delta} +  B^2 \delta D^2  \\
& \leq B^2 d \log (T D ) 
\end{eqnarray*}
 where above $B$ is an upper bound on the function value. 
\end{proof}



==> old-analysis.tex <==
\section{Old Stuff - Only kept to borrow written material}

\subsection{Idealized Online Setting}

Lemma \ref{lemma:approximation_optimal} motivates the use of the following \emph{idealized} online setting. Based on the cost function $c^y_t(\cdot), c^u_t(\cdot)$ and the perturbations $\{w_t\}$, define the following idealized cost of a policy $M$ at time $t$
\ks{need to change cost to match rest of the paper.}
\[ c^{\mathrm{ideal}}_t(M) = c^x_{t+1}(y_{t+1}(M)) + c^u_t(u_t(M))\]
Note that both $x'_{t+1}(M)$ and $u_t(M)$ are affine functions of $M$ and since $c_t^x(\cdot),c^u_t(\cdot)$ are convex functions, we get that $c_t^{ideal}(M)$ is convex in $M$. Using the above we define the following notion of regret which represents the ideal setting. 

\ks{Was there a suggested name for this regret? I like the present one tbh.}
\begin{empheq}[box=\fbox]{align*}
	\;\;\texttt{IdealRegret}(M_0 \ldots M_T) &= \sum_{t=0}^{T} c_t(M_t) - \min_{M_* \in S} c_t(M^*)  \;\;\\
\mathrm{where }\;\; S &= \{M_*^j | \| M_*^j \| \leq \kappa^3(1 - \gamma)^j\}
\end{empheq}

The motivation for the definition of $S$ comes from Lemma \ref{lemma:approximation_optimal} which shows the existence of a spectral norm bound on $M$ to mimic the optimal policy in hindsight. To effectively solve the above problem we define the notion of a slow moving low regret algorithm. Define the movement cost of a sequence $M_1, \ldots M_T$ to be 
\[\textrm{mov}(\{M_0 \ldots M_T\}) = \max_{t \in \{1,T\}} \max_j \|M_t^j - M_{t-1}^j\|\]

We now provide a theorem that shows that a low idealized regret and a low movement cost can be achieved. 

\begin{theorem}
If all the perturbations are bounded by $\|w_t\| \leq \PertBound$, running OGD on the idealized problem produces a sequence of policies $M_1, \ldots M_T$ which have the following properties 
\[ \texttt{IdealRegret}(M_0 \ldots M_T) \leq \frac{2\CostGradBound   \BigBound \PertBound \BBound \kappa^5 d^{3/2} H^{3/2}}{\gamma^{1/2}} \cdot \sqrt{T}\]
\[ \mathrm{mov}(M_0 ... M_T) \leq \frac{2\sqrt{d}\kappa^3\gamma^{-1/2}}{\sqrt{T}}\]
\end{theorem}

\begin{proof}
We first bound the norm of the gradient of the cost $\max_{M \in S}\|\nabla c_t(M)\|$. We first produce a bound on $\|y_t(M)\|$. Using Lemma \ref{lemma:affopnorm} it is immediate seen that 
\begin{equation}
\label{eqn:idealstatebound}
    \|y_t(M)\| \leq \PertBound \cdot \sum_{i=0}^{2\hor}\|\psi_i^K(M)\|  \leq \PertBound \left( \sum_{i=0}^{2\hor} \left(\kappa^2 (1 - \gamma)^i\cdot\mathbf{1}_{i \leq \hor} + 2\hor \cdot  \BBound  \kappa^5 (1 - \gamma)^i\right)\right) \leq \frac{W(\kappa^2 + 2\hor\BBound\kappa^5)}{\gamma}
\end{equation}

We now bound the norm of $\|u_t(M)\|$. Once again by definition we have that 
\[\|u_t(M)\| \leq \|K\|\|y_t(M)\| + \sum_{i=0}^{\hor}\|M^i\|\cdot W \leq \frac{2\PertBound(\kappa^3 + \hor\BBound\kappa^6)}{\gamma}\]
Using Assumption \ref{a2} we now get that \[\max_{M \in S}\|\nabla c_t(M)\| \leq \CostGradBound   \BigBound \PertBound \BBound \kappa^2 d H^{3/2} \]
Further note that the diameter of the set S in $\ell_2$ is at most \[\max_{M_1,M_2 \in S}\|M_1 - M_2\|_F \leq 2\sqrt{d}\kappa^3\gamma^{-1/2} \]
Now using the regret bound from \cite{zinkevich2003online} we get that 
\[ \texttt{IdealRegret} \leq \frac{4 G\PertBound\sqrt{d} \kappa^3(\kappa^3 + \hor\BBound\kappa^6)}{\gamma^{3/2}} \cdot \sqrt{T}\]
The choice of learning rate in OGD also guarantees that
\[ \mathrm{mov}(M_1 \ldots M_T) \leq \frac{2\sqrt{d}\kappa^3\gamma^{-1/2}}{\sqrt{T}}\]
\end{proof}

\na{Put the ONS Regret and Movement Theorem here}

\subsection{Bounding the effect of the movement}

First, for a sequence of policies $M_1, \ldots M_T$, using the movement cost, the following lemma bounds the difference between the actual state $x_t$ played and the ideal state $y_{t+1}(M_t)$. 
\begin{lemma}[State Difference Inequality]
Assuming all perturbations are bounded, i.e. $\|w_t\| \leq \PertBound$
\[ \forall t \;\;\;\; \|x_{t+1} - y_{t+1}(M_t)\| \leq W \cdot \frac{\kappa^2 (1 - \gamma)^\hor + 4\BBound \hor^2 \mathrm{mov}({M_0 \ldots M_T})}{\gamma} + \kappa^2(1 - \gamma)^{\hor+1}\|x_{t-\hor}\|\]
\end{lemma}

\begin{proof}
	Immediately from the definitions we have that 
	\begin{multline*}
		x_{t+1} - y_{t+1}(M_t) =   \sum_{i = 0}^{2\hor}\left( \left((A - BK)^{i} \cdot \mathbf{1}_{i > \hor} + \sum_{j=\max(i - \hor, 1)}^{\min(i, \hor)} (A-BK)^{i-j}B (M_{t - (i - j)}^j - M_t^j) \right) (w_{t-i} + Bc)\right) \\
		 + (A - BK)^{\hor + 1}x_{t-{\hor}}
	\end{multline*}
	and therefore using simple bounds we have that
	\[\|x_{t+1} - y_{t+1}(M_t)\| = W \cdot \frac{\kappa^2 (1 - \gamma)^\hor + 4\BBound \hor^2 \mathrm{mov}({M_0 \ldots M_T})}{\gamma} + \kappa^2(1 - \gamma)^{\hor+1}\|x_{t-\hor}\|\]
% 	\na{From here on we need some inductive proof that $\|x_{t - \hor}\|$ is bounded}
\end{proof}
\begin{proof}
Doing the same derivation as in equation \ref{eqn:idealstatebound} we get that
\[\|x_t\| \leq \frac{W(\kappa^2 + 2\hor\BBound\kappa^5)}{\gamma} + \kappa^2(1 - \gamma)^{\hor}\|x_{t-\hor}\|\]
The above recurrence can be seen to easily satisfy the following upper bound.
\[ \|x_t\| \leq \frac{W(\kappa^2 + 2\hor\BBound\kappa^5)}{\gamma ( 1 - \kappa^2(1 - \gamma)^{\hor})}\]
\end{proof}


\subsection{Relating Total Cost, Regret, Movement Cost and Approximation Cost}

\begin{theorem}
The total regret for Algorithm \ref{alg:ons-lds} is at most
\end{theorem}

\begin{proof}
Before stating the proof we derive a bound on the norm of each of the states $x_t$. Doing the same derivation as in equation \ref{eqn:idealstatebound} we get that
\[\|x_t\| \leq \frac{W(\kappa^2 + 2\hor\BBound\kappa^5)}{\gamma} + \kappa^2(1 - \gamma)^{\hor}\|x_{t-\hor}\|\]
The above recurrence can be seen to easily satisfy the following upper bound.

\begin{equation}
\label{eqn:realstatebound}
    \|x_t\| \leq \BigBound \triangleq  \frac{\PertBound(\kappa^2 + 2\hor\BBound\kappa^5)}{\gamma ( 1 - \kappa^2(1 - \gamma)^{\hor})} 
\end{equation}
Equation \ref{eqn:idealstatebound} shows that 
\begin{equation}
    \|y_t(M_t)\|,\|y_t(M_*)\| \leq \frac{W(\kappa^2 + 2\hor\BBound\kappa^5)}{\gamma} \leq \BigBound
\end{equation}
Ignoring the effect of $M$(by setting it to 0) in the calculation of Equation \ref{eqn:realstatebound}, we get that 
\[\|x_t(K^*)\| \leq \frac{\PertBound\kappa^2}{\gamma ( 1 - \kappa^2(1 - \gamma)^{\hor})} \leq \BigBound\]
Therefore defining 

Consider the following equations. 

\begin{align*}
	&\sum_{t}(c_t^x(x_t) + c_t^u(u_t)) - \left(\min_{K} \sum_{t}(c_t^x(x_t(K)) + c_t^u(u_t(K)))\right) \\ 
	&=\texttt{idealRegret} + \sum_{t}\left(c_t^x(x_t) - c_t^x(y_t(M_t)) \right)+  \sum_t\left(c_t^x(x_t(K^*)) - c_t^x(y_t(M_*))\right) \\
	&\leq\texttt{idealRegret} + \CostGradBound \BigBound \left(\sum_{t}\|x_t - y_t(M_t)\| + \sum_{t}\|x_t(K^*) - y_t(M_*)\| \right) 
\end{align*}
\end{proof}


==> safety.tex <==
\section{Algorithm \& Main Result}

\section{Proof Strategy}
\begin{itemize}
    \item Algorithm - Parameterize policy given $\gamma$ previous noise. Write out state as a linear function $l$ of M. Write out the constraints on $l(M)$. 
    \item Idealized Online Problem - Given $\epsilon_1 ... \epsilon_{\gamma}$ every round. Play a policy $M$, and loss is some function of $l(M)^T\epsilon$. With constraints on $l(M)$. Lets write out a regret bound $R_1$ for this setting. 
    \item Slow moving from above should compare real loss to the above loss. This is achieved by comparing the $x_t^{ideal}$ vs $x_t^{played}$. 
    \item Do the same above for the best policy in hindsight  
\end{itemize}

\subsection{A pertubation-action policy class}
In this section, we put forth the notion of a policy that expresses the recommended action $u_{t+1}$ as a direct function of the past perturbations $w_{t}, \dots w_{1}$.

\ks{Following Sham's suggestion to keep everything -- all $M_t$. Will roll back if I get stuck. I'm dropping the exact mention of the type of norm at all points.}

\begin{definition}
A perturbation-action policy specified by parameters $c,M_1,\dots M_H$ chooses the recommendeded action $u_t$ as
\[ u_{t+1} = c+\sum_{i=0}^{\min\{H, t\}} M_i (w_{t-i}+Bc). \]
\end{definition}

Note that such a policy can be executed because $w_t$ is perfectly determined on the specification of $x_{t+1}$ as $w_t=x_{t+1}-Ax_t-Bu_t$. 

\begin{lemma}\label{l:xonm}
If $u_t$ is chosen as the perturbation-action policy $c, M_1\dots M_H$ recommends, the state sequence is governed by the following law.
\[ x_{t+1} = \sum_{i=0}^t \left(A^{i} + \sum_{j=1}^{\min\{H,i\}} A^{i-j}B M_j\right) (w_{t-i}+Bc) \]
\end{lemma}

We proceed to argue that such a policy class is rich enough to capture the behavior of any strongly stable affine policy class, while guaranteeing that any member of this set has a bounded state \& action sequence.

\begin{lemma}
For any $(\kappa, \gamma)$-strongly stable affine policy $(K,c)$, there exists a perturbation-action policy $c', M_1, \dots M_H$ satisfying the constraints ~\ref{e:cons} for all $i\in [T]$ that produces the same state \& action sequence as the affine policy.
\begin{equation}\label{e:cons} 
\|M_{i+1}\| \leq \kappa^2(1-\gamma)^i \quad ;\quad \left\|A^{i}+ \sum_{j=1}^{i} A^{i-j}B M_j \right \| \leq \kappa (1-\gamma)^{i} \quad ;\quad  \|c'\|\leq \kappa
\|x_t^{ideal} - x_t\| \leq blah 
\end{equation}
Moreover, any perturbation-action policy adhering to equation~\ref{e:cons} produces state \& action sequence $(x_t, u_t)$ with the bounds indicated below for all $t\in [T]$.
\[ \|x_t\| \leq \kappa^3 \gamma^{-1}  \quad ; \quad \|u_t\|\leq \kappa^4\gamma^{-1}.\]
\end{lemma}
\begin{proof}
First, observe the following equalities on the state \& action sequence for an affine controller $(K',c')$.
\[ x_{t+1} = \sum_{i=0}^t(A+BK')^{i}(w_{t-i}+Bc) \quad ; \quad u_{t+1} = c+K'\sum_{i=0}^t(A+BK')^{i}(w_{t-i}+Bc)\]

Now, lemma~\ref{l:xonm} may be used to verify that the choice $c'=c, M_{i+1}=K(A+BK)^{i}$ establishes the first part.

The second part of the claim may be verified independently.
\end{proof}

\subsection{Idealised online setting}
For any policy $\pi$, define $J(\pi|w_0, \dots w_H)$ to be \[J(\pi|w_0\dots w_H) = \sum_{t=0}^H c(x_t, u_t),\] where $x_{t+1}=Ax_t+Bu_t+w_t$ and $u_t=\pi(x_t)$.

Imagine an episodic setting consisting of $T'$ rounds. In each round $t$, the learner declares a perturbation-action policy $\M_t$ and suffers $J(\pi|w_0, \dots w_H)$ for some arbitrarily chosen sequence of $w_0\dots w_H$, which it is thereafter made aware of. The objective of the learner is to minimise the regret defind below.
\[ \texttt{regret}_H = \sum_{t=0}^{T'} J(\pi|w_0, \dots w_H) - \min_{K^*,c^*} \sum_{t=0}^T J((K^*,c^*)|w_0, \dots w_H). \]

The regret minimisation algorithms might be run of a reformulated version of the optimisation problems that is amenable to analysis because it admits reasonable bounds on the gradient norm and diameter. Such a reformulation is stated below.

\begin{lemma}
Define a function $J'(\M|w_0\dots w_H)$ of $\M=(c, M_0\dots M_H)$ as stated below.
\begin{align}\label{e:reform}
    J'(\M|w_0\dots w_H) &= \sum_{t=0}^H c\left(\sum_{i=0}^{t-1} N_i (w_{t-1-i}+Bc), c+\sum_{i=0}^{t-1} M_i (w_{t-1-i}+Bc)\right) \\
    \text{subject to } & N_i = A^i + \sum_{j=1}^i A^{i-j}BM_j \nonumber
\end{align}
Then it must be that $J(\M|w_0\dots w_H)=J'(\M|w_0\dots w_H)$ for any choice of $\M$.
\end{lemma}

\begin{corollary}
Online Gradient Descent when run on the formulation suggested by equation~\ref{e:reform} achieves a regret of $O(G'D'\sqrt{T'})$, where $G'=GH^{\frac{3}{2}}\kappa^6\gamma^{-1}$, $D'=H^{\frac{1}{2}}\kappa^2$. Moreover, if for 2 successive timesteps the policies output by OGD are $\M_t$ amd $\M_{t+1}$ respectively, then $\|\M_t-\M_{t+1}\| \leq \frac{D'}{\sqrt{T}}$.
\end{corollary}

\begin{corollary}
With assumption~\ref{a:sc}, Online Newton Step when run on the formulation suggested by equation~\ref{e:reform} achieves a regret of $O((F'+G'D')d'\log{T'})$, where $G'=GH^{\frac{3}{2}}\kappa^6\gamma^{-1}$, $D'=H^{\frac{1}{2}}\kappa^2$, $F'=LH\kappa^4\gamma^{-1}$, $d=2H$.
\end{corollary}

\ks{These are true, but incomplete. Need a way of saying $\M$ moves slowly. But what definition of slow does theorem 4.7 require? I think we should look at proving 4.7 first.}

\subsection{Online Setting}
We state and prove the main result of the paper in this section.

\begin{theorem}
Judo is ludo.
\end{theorem}

\begin{proof}
We shall use $\M_t$ be the perturbation-action policy played by the regret minimising algorithm at time $t$. 
\begin{align*}
    \texttt{regret} &= J(\A)-J(\K^*,c^*)\\
    &\leq \sum_{t=0}^T \left( J(\M_t|w_{t-H} \dots w_0) - J((K^*,c^*)|w_{t-H} \dots w_0) + \dots\right)
\end{align*}
\end{proof}
